Quantifying the cool ISM in radio AGNs: evidence for late-time re-triggering by galaxy mergers and interactions

We use deep Herschel observations of the complete 2Jy sample of powerful radio AGNs in the local universe (0.05 < z < 0.7) to probe their cool interstellar medium (ISM) contents and star-forming properties, comparing them against other samples of nearby luminous AGNs and quiescent galaxies. This allows us to investigate triggering and feedback mechanisms. We find that the dust masses of the strong-line radio galaxies (SLRGs) in our sample are similar to those of radio-quiet quasars, and that their median dust mass (Mdust = 2 x 10^7 Msun) is enhanced by a factor ~200 compared to that of non-AGN ellipticals, but lower by a factor ~16 relative to that of local ultra-luminous infrared galaxies (UILRGs). Along with compelling evidence for merger signatures in optical images, the SLRGs in our sample also show relatively high star-formation efficiencies, despite the fact that many of them fall below the main sequence for star forming galaxies. Together, these results suggest that most of our SLRGs have been re-triggered by late-time mergers that are relatively minor in terms of their gas contents. In comparison with the SLRGs, the radio AGNs with weak optical emission lines (WLRGs) and edge-darkened radio jets (FRIs) have both lower cool ISM masses and star-formation rates (by a factor of >30), consistent with being fuelled by a different mechanism (e.g. the direct accretion of hot gas).

==> tab4.tex <==
\begin{table*}
\begin{threeparttable}
\caption{Same as Table~\ref{tab:mdustParms} but for the SFRs in $M_\odot$~yr$^{-1}$. The samples of elliptical galaxies were not fit since only constrained by upper limits.\label{tab:SFRParms}}
\centering
\begin{tabular}{ccccc} 
Population &  Samples  &  full sample & SLRGs & WLRGs (FRI/FRII)\\
\hline
\multirow{2}{*}{Radio AGNs} & 2Jy & 3.0$^{\pm1.0}$~(0.3--32.0) & 5.0$^{\pm1.0}$~(0.8--32.0) & \multirow{2}{*}{0.5$^{\pm0.3}$~(0.2--1.0)/0.2$^{\pm0.2}$~(0.0--5.0)} \\\vspace{5pt}
                      & 3CR & 0.5$^{\pm0.3}$~(0.04--6.0) & 0.6$^{\pm0.4}$~(0.0--8.0) & \\
\multirow{2}{*}{QSOs} & PGQs & 2.0$^{\pm0.4}$~(0.3--13.0) & -- & --/-- \\\vspace{5pt}
                      & Type-II & 4.6$^{\pm0.8}$~(0.9--23.0) & -- & --/-- \\\vspace{5pt}
ULIRGs                & HERUS & 109.6$^{\pm17.0}$~(44.0--270.0) & -- & --/--  \\
\multirow{2}{*}{Ellipticals} & Atlas$^{3 \rm D}$ & \multirow{2}{*}{$<~0.01$} & \multirow{2}{*}{--} & \multirow{2}{*}{--/--}  \\\vspace{5pt}
                      &  HRS  & &  & \\
\end{tabular}%
\end{threeparttable}
\end{table*}

